An obstruction to subfactor principal graphs from the graph planar algebra embedding theorem

We find a new obstruction to the principal graphs of subfactors. It shows that in a certain family of 3-supertransitive principal graphs, there must be a cycle by depth 6, with one exception, the principal graph of the Haagerup subfactor.

==> documentclasshack.tex <==
%auto-ignore
%%%%%% a hack to make the documentclass name available later %%%
% Thanks to Morten Høgholm. I stole this code from 
% http://groups.google.com/group/comp.text.tex/msg/142306cc7f8acdac
\let\LaTeXdocumentclass\documentclass
\renewcommand*\documentclass[2][]{%
   \newcommand*\ClassName{#2}% for later use
   \LaTeXdocumentclass[#1]{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> text/top_matter.tex <==
%!TEX root = ../obstruction.tex

\title{Obstructions to subfactor principal graphs from the graph planar algebra embedding theorem}

\author{Scott~Morrison}
\address{
}%
\email{scott@tqft.net}

\address{%
\rm URL:\stdspace \tt \url{http://tqft/net/}}


\date{
  First edition: the mysterious future
  This edition: \today.
}

\primaryclass{} \secondaryclass{} \keywords{
}

